Axiomatic Construction of Hierarchical Clustering in Asymmetric Networks

This paper considers networks where relationships between nodes are represented by directed dissimilarities. The goal is to study methods for the determination of hierarchical clusters, i.e., a family of nested partitions indexed by a connectivity parameter, induced by the given dissimilarity structures. Our construction of hierarchical clustering methods is based on defining admissible methods to be those methods that abide by the axioms of value - nodes in a network with two nodes are clustered together at the maximum of the two dissimilarities between them - and transformation - when dissimilarities are reduced, the network may become more clustered but not less. Several admissible methods are constructed and two particular methods, termed reciprocal and nonreciprocal clustering, are shown to provide upper and lower bounds in the space of admissible methods. Alternative clustering methodologies and axioms are further considered. Allowing the outcome of hierarchical clustering to be asymmetric, so that it matches the asymmetry of the original data, leads to the inception of quasi-clustering methods. The existence of a unique quasi-clustering method is shown. Allowing clustering in a two-node network to proceed at the minimum of the two dissimilarities generates an alternative axiomatic construction. There is a unique clustering method in this case too. The paper also develops algorithms for the computation of hierarchical clusters using matrix powers on a min-max dioid algebra and studies the stability of the methods proposed. We proved that most of the methods introduced in this paper are such that similar networks yield similar hierarchical clustering results. Algorithms are exemplified through their application to networks describing internal migration within states of the United States (U.S.) and the interrelation between sectors of the U.S. economy.

==> proof_theo_extended_value.tex <==
%!TEX root = Asymmetric_Clustering_Journal_V_current.tex

\begin{myproof}[of Theorem \ref{theo_extended_value}]
In proving Theorem \ref{theo_extended_value}, we make use of the following lemma which proves that, given a network, if the directed minimum chain cost $\tdu^*_X(x, x') \geq \delta$ between $x, x' \in X$ is at least $\delta$ it is possible to find a network partition separating $x$ and $x'$ such that the dissimilarities between points in different partitions are bounded below by $\delta$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{lemma_axiom_redundancy}
Let $N=(X, A_X)$ be any network and $\delta$ any positive constant. Suppose that $x,x' \in X$ are such that their associated minimum chain cost [cf. \eqref{eqn_nonreciprocal_chains}] satisfies
%
\begin{align}\label{eqn_lem_axiom_redundancy_01} 
   \tdu^*_X(x, x') \geq \delta.
\end{align} 
%
Then, there exists a partition $P_\delta(x,x')=\{B_\delta(x), B_\delta(x')\}$ of the node space $X$ into blocks $B_\delta(x)$ and $B_\delta(x')$ with $x \in B_\delta(x)$ and $x' \in B_\delta(x')$ such that for all points $b \in B_\delta(x)$ and $b' \in B_\delta(x')$
%
\begin{align}\label{eqn_lem_axiom_redundancy_02} 
   A_X(b, b') \geq \delta.
\end{align} \end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproofnoname}
We prove this result by contradiction. If a partition $P_\delta(x,x')=\{B_\delta(x), B_\delta(x')\}$ with $x \in B_\delta(x)$ and $x' \in B_\delta(x)$ satisfying \eqref{eqn_lem_axiom_redundancy_02} does not exist for all pairs of points $x,x'\in X$ satisfying \eqref{eqn_lem_axiom_redundancy_01}, then there is at least one pair of nodes $x,x'\in X$ satisfying \eqref{eqn_lem_axiom_redundancy_01} such that for {\it all} partitions of $X$ into two blocks $P=\{B, B'\}$ with $x \in B$ and $x' \in B'$ we can find at least a pair of elements $b_P \in B$ and $b'_P \in B'$ for which
%
\begin{equation}\label{eqn_lem_axiom_redundancy_03} 
   A_X(b_P, b'_P) < \delta.
\end{equation}
%
Begin by considering the partition $P_1=\{B_1, B'_1\}$ where $B_1 = \{ x \}$ and $B'_1 = X \backslash \{x\}$. Since \eqref{eqn_lem_axiom_redundancy_03} is true for all partitions having $x\in B$ and $x'\in B'$ and $x$ is the unique element of $B_1$, there must exist a node $b'_{P_1} \in B'_1$ such that  
%
\begin{equation}\label{eqn_lem_axiom_redundancy_04} 
   A_X(x, b'_{P_1}) <  \delta. 
\end{equation}
%
Hence, the chain $C(x, b'_{P_1})= [x, b'_{P_1}]$ composed of these two nodes has cost smaller than $\delta$. Moreover, since $\tdu^*_X(x, b'_{P_1})$ represents the minimum cost among all chains $C(x, b'_{P_1})$ linking $x$ to $b'_{P_1}$, we can assert that
%
\begin{equation}\label{eqn_lem_axiom_redundancy_04_1} 
   \tdu^*_X(x, b'_{P_1}) \leq  A_X(x, b'_{P_1}) <  \delta.
\end{equation}
%
Consider now the partition $P_2=\{B_2, B'_2\}$ where $B_2= \{ x, b'_{P_1} \}$ and $B'_2=X \backslash B_2$. From \eqref{eqn_lem_axiom_redundancy_03}, there must exist a node $b'_{P_2} \in B'_2$ that satisfies at least one of the two following conditions 
%
\begin{align}
   &A_X(x, b'_{P_2}) <  \delta,  \label{eqn_lem_axiom_redundancy_05} \\
   &A_X(b'_{P_1}, b'_{P_2}) <  \delta. \label{eqn_lem_axiom_redundancy_06}
\end{align}
%
If \eqref{eqn_lem_axiom_redundancy_05} is true, the chain $C(x, b'_{P_2})=[x, b'_{P_2}]$ has cost smaller than $\delta$. If \eqref{eqn_lem_axiom_redundancy_06} is true, we combine the dissimilarity bound  with the one in \eqref{eqn_lem_axiom_redundancy_04} to conclude that the chain $C(x, b'_{P_2})=[x, b'_{P_1}, b'_{P_2}]$ has cost smaller than $\delta$. In either case we conclude that there exists a chain $C(x, b'_{P_2})$ linking $x$ to $b'_{P_2}$ whose cost is smaller than $\delta$. Therefore, the minimum chain cost must satisfy
%
\begin{equation}\label{eqn_lem_axiom_redundancy_04_2} 
\tdu^*_X(x, b'_{P_2}) <  \delta.
\end{equation}
%
Repeat the process by considering the partition $P_3$ with $B_3= \{ x, b'_{P_1}, b'_{P_2} \}$ and $B'_3=X\backslash B_3$. As we did in arguing \eqref{eqn_lem_axiom_redundancy_05}-\eqref{eqn_lem_axiom_redundancy_06} it must follow from \eqref{eqn_lem_axiom_redundancy_03} that there exists a point $b'_{P_3}$ such that at least one of the dissimilarities $A_X(x, b'_{P_3})$, $A_X(b'_{P_1}, b'_{P_3})$, or $A_X( b'_{P_2}, b'_{P_3})$ is smaller than $\delta$. This observation implies that at least one of the chains $[x, b'_{P_3}]$, $[x, b'_{P_1}, b'_{P_3}]$, $[x, b'_{P_2}, b'_{P_3}]$, or $[x, b'_{P_1}, b'_{P_2}, b'_{P_3}]$ has cost smaller than $\delta$ from where it follows
%
\begin{equation}\label{eqn_lem_axiom_redundancy_04_3} 
   \tdu^*_X(x, b'_{P_3}) <  \delta.
\end{equation}
%
This recursive construction can be repeated $n-1$ times to obtain partitions $P_1, P_2, ... , P_{n-1}$ and corresponding nodes $b'_{P_1}, b'_{P_2}, \dots, b'_{P_{n-1}}$ such that the minimum chain cost satisfies
%
\begin{equation}\label{eqn_lem_axiom_redundancy_04_4} 
   \tdu^*_X(x, b'_{P_i}) <  \delta, \qquad \text{for all\ } i.
\end{equation}
%
Observe that nodes $b'_{P_i}$ are distinct by construction and distinct from $x$. Since there are $n$ nodes in the network it must be that $x'=b'_{P_k}$ for some $i \in \{1, \ldots , n-1\}$. It follows from \eqref{eqn_lem_axiom_redundancy_04_4} that
%
\begin{equation}\label{eqn_lem_axiom_redundancy_04_5} 
\tdu^*_X(x, x') <  \delta.
\end{equation}
%
This is a contradiction because $x,x'\in X$ were assumed to satisfy \eqref{eqn_lem_axiom_redundancy_01}. Thus, the assumption that \eqref{eqn_lem_axiom_redundancy_03} is true for {\it all} partitions is incorrect. Hence, the claim that there is a partition $P_\delta(x,x')=\{B_\delta(x), B_\delta(x')\}$ satisfying \eqref{eqn_lem_axiom_redundancy_02} must be true. \end{myproofnoname}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\noindent
Continuing with the main proof of Theorem \ref{theo_extended_value}, to prove that (A1)-(A2) imply (A1')-(A2) let $\ccalH$ be a method that satisfies (A1) and (A2) and denote by $(\{1, 2, \ldots, n\},u_{n, \alpha, \beta})= \ccalH(\vec{\Delta}_n(\alpha,\beta,\Pi))$ the output ultrametric resulting of applying $\ccalH$ to the network $\vec{\Delta}_n(\alpha,\beta,\Pi)$ considered in the Extended Axiom of Value (A1'). We want to prove that (A1') is satisfied which means that we have to show that for all indices $n\in\mbN$, constants $\alpha,\beta>0$, permutations $\Pi$ of $\{1,\ldots,n\}$, and points $i\neq j$, we have $u_{n, \alpha, \beta}(i,j)=\max(\alpha,\beta)$. We will do so by showing both
%
\begin{align}
   &u_{n, \alpha, \beta}(i,j)\ \leq\ \max(\alpha,\beta)  \label{eqn_lem_axiom_redundancy_001}, \\
   &u_{n, \alpha, \beta}(i,j)\ \geq\ \max(\alpha,\beta)  \label{eqn_lem_axiom_redundancy_002},
\end{align}
%
for all $n\in\mbN$, $\alpha,\beta>0$, $\Pi$, and $i\neq j$.

To prove \eqref{eqn_lem_axiom_redundancy_001} define a symmetric two-node network $\vec{\Delta}_2(\max(\alpha, \beta), \max(\alpha, \beta))=(\{p,q\}, A_{p,q})$ where $A_{p,q}(p,q)=A_{p,q}(q,p)=\max(\alpha, \beta)$ and denote by $\big(\{p, q\}, u_{p,q}\big)=\ccalH(\vec{\Delta}_2(\max(\alpha, \beta), \max(\alpha, \beta)))$ the outcome of method $\ccalH$ when applied to $\vec{\Delta}_2(\max(\alpha, \beta), \max(\alpha, \beta))$. Since the method $\ccalH$ abides by (A1),
%
\begin{align}\label{eqn_lem_axiom_redundancy_110}
   u_{p,q}(p,q)
      = \max\big(\max(\alpha, \beta),\max(\alpha, \beta)\big)
      = \max(\alpha, \beta).
\end{align}
%
Consider now the map $\phi_{i,j}:\{p,q\} \to \{1,\ldots,n\}$ from the two-node network $\vec{\Delta}_2(\max(\alpha, \beta), \max(\alpha, \beta))$ to the permuted canonical network $\vec{\Delta}_n(\alpha,\beta,\Pi)$ where $\phi_{i,j}(p)=i$ and $\phi_{i,j}(q)=j$. Since dissimilarities in $\vec{\Delta}_n(\alpha,\beta,\Pi)$ are either $\alpha$ or $\beta$ and the dissimilarities in $\vec{\Delta}_2(\max(\alpha, \beta), \max(\alpha, \beta))$ are $\max(\alpha,\beta)$ it follows that the map $\phi_{i,j}$ is dissimilarity reducing regardless of the particular values of $i$ and $j$. Since the method $\ccalH$ was assumed to satisfy (A2) as well, we must have 
%
\begin{align}\label{eqn_lem_axiom_redundancy_120}
   u_{p,q} (p,q) 
      \geq  u_{n, \alpha, \beta}\big(\phi_{i,j}(p),\phi_{i,j}(q)\big) 
      =     u_{n, \alpha, \beta}(i,j) .
\end{align}
%
The inequality in \eqref{eqn_lem_axiom_redundancy_001} follows form substituting \eqref{eqn_lem_axiom_redundancy_110} into \eqref{eqn_lem_axiom_redundancy_120}.

In order to show inequality \eqref{eqn_lem_axiom_redundancy_002}, pick two arbitrary distinct nodes $i, j \in \{1,\ldots,n\}$ in the node set of $\vec{\Delta}_n(\alpha,\beta,\Pi)$. Denote by $C(i,j)$ and $C(j,i)$ two minimizing chains in the definition  \eqref{eqn_nonreciprocal_chains} of the directed minimum chain costs $\tdu^*_{n, \alpha, \beta}(i, j)$ and $\tdu^*_{n, \alpha, \beta}(j, i)$ respectively. Observe that at least one of the following two inequalities must be true
%
\begin{align}
   \tdu^*_{n, \alpha, \beta}(i, j) \geq \max(\alpha, \beta), \label{eqn_inequality_max_i_j} \\
   \tdu^*_{n, \alpha, \beta}(j, i) \geq \max(\alpha, \beta). \label{eqn_inequality_max_j_i}
\end{align}
%
Indeed, if both \eqref{eqn_inequality_max_i_j} and \eqref{eqn_inequality_max_j_i} were false, the concatenation of $C(i,j)$ and $C(j,i)$ would form a loop $C(i,i)=C(i,j) \uplus C(j,i)$ of cost strictly less than $\max(\alpha, \beta)$. This cannot be true because $\max(\alpha, \beta)$ is the minimum loop cost of the network  $\vec{\Delta}_n(\alpha,\beta,\Pi)$ as we already showed in \eqref{eqn_mlc_extended_value}.



Without loss of generality assume \eqref{eqn_inequality_max_i_j} is true and consider $\delta = \max(\alpha, \beta)$. By Lemma \ref{lemma_axiom_redundancy} we are therefore guaranteed to find a partition of the node set $\{1,\ldots,n\}$ into two blocks $B_\delta(i)$ and $B_\delta(j)$  with $i \in B_\delta(i)$ and $j \in B_\delta(j)$ such that for all $b \in B_\delta(i)$ and $b' \in B_\delta(j)$ it holds that 
%
\begin{equation}\label{eqn_b_bprime_max}
   \Pi(A_{n,\alpha,\beta})(b, b') \geq \delta = \max(\alpha, \beta).
\end{equation}
%
Define a two-node network $\vec{\Delta}_2(\max(\alpha, \beta), \min(\alpha, \beta))=(\{r, s\}, A_{r,s})$ where $A_{r,s}(r,s)=\max(\alpha, \beta)$ and $A_{r,s}(s,r)=\min(\alpha, \beta)$ and denote by $(\{r,s\},u_{r,s})=\ccalH(\vec{\Delta}_2(\max(\alpha, \beta), \min(\alpha, \beta)))$. Since the method $\ccalH$ satisfies (A1) we must have
%
\begin{equation}\label{eqn_max_max_min_a_b}
   u_{r,s}(r, s)
      = \max \big( \max(\alpha, \beta), \min(\alpha, \beta) \big) 
      = \max(\alpha, \beta).
\end{equation}
%
Consider the map $\phi'_{i,j} : \{1,\ldots,n\} \to \{r, s\}$ such that $\phi'_{i,j}(b)=r$ for all $b \in B_\delta(i)$ and $\phi'_{i,j}(b')=s$ for all $b' \in B_\delta(j)$. The map $\phi'_{i,j}$ is dissimilarity reducing because
%
\begin{equation}\label{eqn_phi_dissim_reducing_i_j}
      \Pi(A_{n,\alpha,\beta})(k,l) \geq A_{r,s}(\phi'_{i,j}(k), \phi'_{i,j}(l)),
\end{equation}
%
for all $k, l \in \{1,\ldots,n\}$. To see the validity of \eqref{eqn_phi_dissim_reducing_i_j} consider three different possible cases. If $k$ and $l$ belong both to the same block, i.e., either $k,l \in B_\delta(i)$ or $k,l \in B_\delta(j)$, then $\phi'_{i,j}(k)=\phi'_{i,j}(l)$ and $A_{r,s}(\phi'_{i,j}(k), \phi'_{i,j}(l))=0$ which cannot exceed the nonnegative $\Pi(A_{n,\alpha,\beta})(k,l)$. If $k \in B_\delta(j)$ and $l \in B_\delta(i)$ it holds that $A_{r,s}(\phi'_{i,j}(k), \phi'_{i,j}(l)) = A_{r,s}(s, r)= \min(\alpha, \beta)$ which cannot exceed $\Pi(A_{n,\alpha,\beta})(k,l)$ which is either equal to $\alpha$ or $\beta$. If $k \in B_\delta(i)$ and $l \in B_\delta(j)$, then we have $A_{r,s}(\phi'_{i,j}(k), \phi'_{i,j}(l)) = A_{r,s}(r, s)= \max(\alpha, \beta)$ but we also have $\Pi(A_{n,\alpha,\beta})(k,l)= \max(\alpha, \beta)$ as it follows by taking $b=k$ and $b'=l$ in \eqref{eqn_b_bprime_max}.

Since $\ccalH$ satisfies the Axiom of Transformation (A2) and the map $\phi'_{i,j}$ is dissimilarity reducing we must have
%
\begin{equation}\label{eqn_phi_dissim_reducing_i_j_2}
   u_{n, \alpha, \beta}(i,j) \geq u_{r,s}\big(\phi'_{i,j}(i), \phi'_{i,j}(j)\big) = u_{r,s}(r, s).
\end{equation}
%
Substituting \eqref{eqn_max_max_min_a_b} in \eqref{eqn_phi_dissim_reducing_i_j_2} we obtain the inequality \eqref{eqn_lem_axiom_redundancy_002}. Combining this result with the validity of \eqref{eqn_lem_axiom_redundancy_001}, it follows that $u_{n, \alpha, \beta}(i,j)= \max(\alpha,\beta)$ for all $n\in\mbN$, $\alpha,\beta>0$, $\Pi$, and $i\neq j$. Thus, admissibility with respect to (A1)-(A2) implies admissibility with respect to (A1')-(A2). That admissibility with respect to (A1')-(A2) implies admissibility with respect to (A1)-(A2) is immediate because (A1) is a particular case of (A1'). Hence, if a method satisfies axioms (A1') and (A2) it must satisfy (A1) and (A2). The stated equivalence between admissibility with respect to (A1)-(A2) and (A1')-(A2) follows. \end{myproof}

==> proof_theo_influence_redundancy.tex <==
%!TEX root = Asymmetric_Clustering_Journal_V_current.tex

\begin{myproof}[of Theorem \ref{theo_influence_redundancy}]
The following lemma is instrumental towards the proof of Theorem \ref{theo_influence_redundancy}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{lemma_influence_redundancy}
Let $N=(X, A_X)$ be an arbitrary network with $n$ nodes and $\vec{\Delta}_n(\alpha,\beta)=(\{1,\ldots,n\}, A_{n,\alpha,\beta})$ be the canonical network in \eqref{eqn_extended_axiom_of_value_canonical_matrix} with $0 < \alpha \leq \sep(X, A_X)$ [cf. \eqref{eqn_def_separation_network}] and $\beta=\mlc(X, A_X)$ [cf. \eqref{eqn_def_mlc}]. Then, there exists a bijective map $\phi:X\to\{1,\ldots,n\}$ such that
%
\begin{align}\label{eqn_dissim_m_3}
   A_X(x, x') \geq A_{n, \alpha,\beta}(\phi(x), \phi(x')),
\end{align}
for all $x, x' \in X$.
 \end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproofnoname} To construct the map $\phi$ consider the function $P:X \to \mathcal{P}(X)$ from the node set $X$ to its power set $\mathcal{P}(X)$ such that
%
\begin{equation}\label{eqn_function_predecessor}
   P(x) :=\{ x' \in X \, | \, x' \neq x \,\, , \,\, A_X(x', x)<\beta\},
\end{equation} 
%
for all $x \in X$.
Having $r \in P(s)$ for some $r,s \in X$ implies that $A_X(r, s) < \beta=\mlc(X,A_X)$. An important observation is that we must have a node $x\in X$ whose $P$-image is empty. Otherwise, pick a node $x_n\in X$ and construct the chain $[x_0, x_1, \ldots , x_n]$ where the $i$th element of the chain $x_{i-1}$ is in the $P$-image of $x_i$. From the definition of the map $P$ it follows that all dissimilarities along this chain satisfy $A_X(x_{i-1},x_{i})<\beta=\mlc(X,A_X)$. But since the chain $[x_0, x_1, \ldots , x_n]$ contains $n+1$ elements, at least one node must be repeated. Hence, we have found a loop for which all dissimilarities are bounded above by $\beta=\mlc(X,A_X)$, which is impossible because it contradicts the definition of the minimum loop cost in \eqref{eqn_def_mlc}.  We can then find a node $x_{i_1}$ for which $P(x_{i_1})=\emptyset$. Fix $\phi(x_{i_1})=1$. 

Select now a node $x_{i_2}\neq x_{i_1}$ whose $P$-image is either $\{x_{i_1}\}$ or $\emptyset$, which we write jointly as $P(x_{i_2}) \subseteq \{x_{i_1}\}$. Such a node must exist, otherwise, pick a node $x_{n-1}\in X\backslash \{x_{i_1}\}$ and construct the chain $[x_0, x_1, \ldots , x_{n-1}]$ where $x_{i-1} \in P(x_i) \backslash \{x_{i_1}\}$, i.e. $x_{i-1}$ is in the $P$-image of $x_i$ and $x^{i-1} \neq \{x_{i_1}\}$. Since the chain $[x_0, x_1, ... , x_{n-1}]$ contains $n$ elements from the set $X\backslash \{x_{i_1}\}$ of cardinality $n-1$, at least one node must be repeated. Hence, we have found a loop where all dissimilarities between consecutive nodes satisfy $A_X(x^{i-1},x^{i})<\beta=\mlc(X,A_X)$, contradicting the definition of minimum loop cost. We can then find a node $x_{i_2} \neq x_{i_1}$ for which $P(x_{i_2}) \subseteq \{x_{i_1}\}$. Fix $\phi(x_{i_2})=2$.

Repeat this process $k$ times so that at step $k$ we have $\phi(x_{i_k})=k$ for a node $x_{i_k} \not\in \{x_{i_1},x_{i_2},\ldots x_{i_{k-1}}\}$ whose P-image is a subset of the nodes already picked, that is
%
\begin{equation}
   P(x_{i_k}) \subseteq \{x_{i_1},x_{i_2},\ldots x_{i_{k-1}}\}.
\end{equation}
%
This node must exist, otherwise, we could start with a node $x_{n-k+1} \in X \backslash \{x_{i_1},x_{i_2},\ldots x_{i_{k-1}}\}$ and construct a chain $[x_0, x_1, \ldots , x_{n-k+1}]$ where $x_{i-1} \in P(x_i) \backslash \{x_{i_1},x_{i_2},\ldots x_{i_{k-1}}\}$ and arrive to the same contradiction as for the case $k=2$.

Since all the nodes $x_{i_k}$ are different, the map $\phi$ with $\phi(x_{i_k})=k$ is bijective. By construction, $\phi$ is such that for all $l>k$, $x_{i_l}\notin P(x_{i_k})$. From \eqref{eqn_function_predecessor}, this implies that the dissimilarity from $x_{i_l}$ to $x_{i_k}$ must satisfy
%
\begin{equation}\label{eqn_dissim_m_1}
   A_X(x_{i_l},x_{i_k}) \geq \beta, \qquad \text{for all\ } l>k.
\end{equation} 
%
Moreover, from the definition of the canonical matrix $A_{n, \alpha,\beta}$ in \eqref{eqn_extended_axiom_of_value_canonical_matrix} we have that for $l>k$
%
\begin{equation}\label{eqn_dissim_m_2}
   A_{n, \alpha,\beta}(\phi(x_{i_l}), \phi(x_{i_k})) 
      = A_{n, \alpha,\beta}(l,k)    
      = \beta.
\end{equation}
%
By comparing \eqref{eqn_dissim_m_2} with \eqref{eqn_dissim_m_1} we conclude that \eqref{eqn_dissim_m_3} is true for all points with $\phi(x)>\phi(x')$. When $\phi(x)<\phi(x')$, we have $A_{n, \alpha,\beta}(\phi(x), \phi(x'))=\alpha$ which was assumed to be bounded above by the separation of the network $(X, A_X)$, thus, $A_{n, \alpha,\beta}(\phi(x), \phi(x'))$ is not greater than any positive dissimilarity in the range of $A_X$.
\end{myproofnoname}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\noindent
Continuing the main proof of Theorem \ref{theo_influence_redundancy}, consider a given arbitrary network $N=(X, A_X)$ with $X=\{x_1, x_2, ... , x_n\}$ and denote by $(X, u_X)=\ccalH(X,A_X)$ the output of applying the clustering method $\ccalH$ to the network $N$. The method $\ccalH$ is known to satisfy (A1') and (A2) and we want to show that it satisfies (P1) for which we need to show that $u_X(x,x')\geq\mlc(X,A_X)$ for all $x\neq x'$ [cf. \eqref{eqn_mlc_lowerbounds_ultrametric}]. 

Consider the canonical network $\vec{\Delta}_n(\alpha,\beta)=(\{1,\ldots,n\}, A_{n,\alpha,\beta})$ in \eqref{eqn_extended_axiom_of_value_canonical_matrix} with $\beta=\mlc(X, A_X)$ being the minimum loop cost of the network $N$ [cf. \eqref{eqn_def_mlc}] and $\alpha>0$ a constant not exceeding the separation of the network \eqref{eqn_def_separation_network}. Thus, we have $\alpha\leq\sep(X,A_X)\leq\mlc(X,A_X)=\beta$. Note that networks $N$ and $\vec{\Delta}_n(\alpha,\beta)$ have equal number of nodes. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F       C   O   N   T   I   N   U   E   D   %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Denote by $(\{1,\ldots,n\}, u_{\alpha,\beta}) = \ccalH(\vec{\Delta}_n(\alpha,\beta))$ the ultrametric space obtained when we apply the clustering method $\ccalH$ to the network $\vec{\Delta}_n(\alpha,\beta)$. Since $\ccalH$ satisfies the Extended Axiom of Value (A1'), then for all indices $i, j \in \{1,\ldots,n\}$ with $i \neq j$ we have
%
\begin{equation}\label{eqn_ultram_epsilon_m_1}
   u_{\alpha,\beta}(i,j) = \max(\alpha,\beta) = \beta = \mlc(X,A_X) .
\end{equation}
%
Further, focus on the bijective dissimilarity reducing map considered in Lemma \ref{lemma_influence_redundancy} and notice that since the method $\ccalH$ satisfies the Axiom of Transformation (A2) it follows that for all $x, x' \in X$ 
%
\begin{equation}\label{eqn_ultram_epsilon_m_2}
u_X(x,x') \geq u_{\alpha,\beta}(\phi(x), \phi(x')).
\end{equation}
%
Since the equality in \eqref{eqn_ultram_epsilon_m_1} is true for all $i\neq j$ and since all points $x\neq x'$ are mapped to points $\phi(x)\neq\phi(x')$ because $\phi$ is bijective, \eqref{eqn_ultram_epsilon_m_2} implies
%
\begin{equation}\label{eqn_ultram_epsilon_m_3}
   u_X(x,x') \geq \beta = \mlc(X, A_X),
\end{equation}
%
for all distinct $x, x' \in X$. This is the definition of the Property of Influence (P1). 
\end{myproof}
